Data Assimilation for hyperbolic conservation laws. A Luenberger observer approach based on a kinetic description

Developing robust data assimilation methods for hyperbolic conservation laws is a challenging subject. Those PDEs indeed show no dissipation effects and the input of additional information in the model equations may introduce errors that propagate and create shocks. We propose a new approach based on the kinetic description of the conservation law. A kinetic equation is a first order partial differential equation in which the advection velocity is a free variable. In certain cases, it is possible to prove that the nonlinear conservation law is equivalent to a linear kinetic equation. Hence, data assimilation is carried out at the kinetic level, using a Luenberger observer also known as the nudging strategy in data assimilation. Assimilation then resumes to the handling of a BGK type equation. The advantage of this framework is that we deal with a single "linear" equation instead of a nonlinear system and it is easy to recover the macroscopic variables. The study is divided into several steps and essentially based on functional analysis techniques. First we prove the convergence of the model towards the data in case of complete observations in space and time. Second, we analyze the case of partial and noisy observations. To conclude, we validate our method with numerical results on Burgers equation and emphasize the advantages of this method with the more complex Saint-Venant system.

==> frontmatter.tex <==
%!TEX root = BMPS_article.tex

\title[Data Assimilation for hyperbolic conservation laws]{Data Assimilation for hyperbolic conservation laws. \\A Luenberger observer approach based on a kinetic description}

%An observer approach based on a kinetic description

\author{A.-C.~Boulanger}
   \address{UPMC, CNRS UMR 7598,  Laboratoire Jacques-Louis  Lions, F-75005, Paris and INRIA Rocquencourt EPI ANGE}
   \email{anne-celine.boulanger@inria.fr}
\author{P.~Moireau}
   \address{INRIA Saclay EPI M3DISIM}
\author{B.~Perthame}
   \address{UPMC, CNRS UMR 7598,  Laboratoire Jacques-Louis  Lions, F-75005, Paris and INRIA Rocquencourt EPI BANG}
\author{J.~Sainte-Marie}
   \address{INRIA Rocquencourt EPI ANGE and CETMEF, 2 Boulevard
  Gambetta, 60200 Compi\`egne}


\begin{abstract}
Developing robust data assimilation methods for hyperbolic conservation laws is a challenging subject. Those PDEs indeed show no dissipation effects and the input of additional information in the model equations may introduce errors that propagate and create shocks.
% Besides, in the nonlinear case, usual techniques such as sequential methods (Kalman filter) or \tochange{variational methods (4D-VAR) admit no convergence proofs}.
We propose a new approach based on the kinetic description of the conservation law. A kinetic equation is a first order partial differential equation in which the advection velocity is a free variable. In certain cases, it is possible to prove that the nonlinear conservation law is equivalent to a linear kinetic equation. Hence, data assimilation is carried out at the kinetic level, using a Luenberger observer also known as the nudging strategy in data assimilation. Assimilation then resumes to the handling of a BGK type equation. The advantage of this framework is that we deal with a single ``linear'' equation instead of a nonlinear system and it is easy to recover the macroscopic variables. 
The study is divided into several steps and essentially based on functional analysis techniques. First we prove the convergence of the model towards the data in case of complete observations in space and time. Second, we analyze the case of partial and noisy observations. To conclude, we validate our method with numerical results on Burgers equation and emphasize the advantages of this method with the more complex Saint-Venant system.
\end{abstract}

% AMS subject classifications (used in AMS journals)
\subjclass{35L40, 35L65, 65M08, 76D55, 93E11}

% AMS keywords (used in AMS journals)
\keywords{Data assimilation, hyperbolic conservation law, kinetic formulation, nudging, shallow water system}


\maketitle
